Vertical Federated Learning: Concepts, Advances and Challenges

Vertical Federated Learning (VFL) is a federated learning setting where multiple parties with different features about the same set of users jointly train machine learning models without exposing their raw data or model parameters. Motivated by the rapid growth in VFL research and real-world applications, we provide a comprehensive review of the concept and algorithms of VFL, as well as current advances and challenges in various aspects, including effectiveness, efficiency, and privacy. We provide an exhaustive categorization for VFL settings and privacy-preserving protocols and comprehensively analyze the privacy attacks and defense strategies for each protocol. In the end, we propose a unified framework, termed VFLow, which considers the VFL problem under communication, computation, privacy, as well as effectiveness and fairness constraints. Finally, we review the most recent advances in industrial applications, highlighting open challenges and future directions for VFL.

==> application.tex <==
\section{Applications}
\label{applied}
%\subsection{Industrial Applications}
Due to its practical merits for enabling data  collaboration between multiple institutions across industries, VFL has attracted increasing attention from both academia and industry, especially since the rising privacy concerns over data collection has led to the enforcement of strict regulations such as GDPR. Privacy-preserving platforms and open-sourced projects, industrial standardization as well as use cases have flourished in recent years. In this section, we provide an overview of VFL projects, standards, and applications.

\subsection{Software and open-sourced projects}
In recent years, we have witnessed the rapid development of federated learning projects and platforms by academia and industry, such as Google's TensorFlow Federated (TFF)\cite{bonawitz2019towards}, Webank's FATE\cite{liu2021fate}, OpenMined's Pysyft\cite{ryffel2018generic,romanini2021pyvertical}, FedML\cite{he2020fedml}, Baidu's PaddleFL\cite{PaddleFL}, ByteDance's Fedlearner\cite{Fedlearner}, Alibaba's FederatedScope\cite{xie2022federatedscope},and the FedTree\cite{fedtree2022} framework jointly proposed by National University of Singapore and Tsinghua University. A majority of these frameworks, including FATE, Fedlearner, PaddleFL, Pysyft, FedTree, and FedML  support VFL and cross-silo collaborative learning.  

FATE is an open-sourced project initiated by WeBank in 2019 which is the first industrial-grade FL platform that supports a variety of horizontal, vertical and federated transfer learning algorithms; PyVertical\cite{romanini2021pyvertical}, developed by the OpenMined community, is a privacy-preserving deep learning library that supports vertical federated learning ; FedML is an open research library for research-oriented FL development that supports simulation-scale of VFL; PaddleFL, open sourced by Baidu, is an open-source federated learning framework based on PaddlePaddle, supporting a variety of horizontal and vertical federated learning algorithms and CV and NLP applications; Fedlearner is open-sourced by ByteDance, focusing on vertical federated learning algorithms and their applications in the recommendation field; FedTree was proposed by researchers from National University of Singapore and Tsinghua University. It is a federated learning system which focuses on training tree models and supports vertical federated learning; FederatedScope, developed by Alibaba, is another federated learning platform that supports horizontal, vertical federated learning and Graph-based Personalized Federated Learning. Alimama has open-sourced the Elastic-Federated-Learning-Solution (EFLS) project, which is mainly aimed at two-party vertical federated learning scenarios \cite{EFLS2022}.

\subsection{Standardization}
Through the establishment of standard development working groups under the major organizations such as IEEE (Institute of Electrical and Electronics Engineers), ITU (International Telecommunication Union), 3GPP (3rd Generation Partnership Project), ETSI (European Telecommunications Standards Institute), CCSA (China Communications Standards Association) ),  a series of standardization work has been carried out for the concept, framework and requirements of federated learning technology. 

The earliest federated learning standard is IEEE p3652.1 “guide for architectural framework and application of Federated machine learning”, which was initiated and developed by Webank in December 2018. This standard defines the federated machine learning framework, federated learning into horizontal federated learning, vertical federated learning, and federated transfer learning from the perspective of data overlap, Reference examples of vertical federated are given in detail. The standard was officially approved in March 2021. %\yang{add a few sentences on VFL covered in this standard}

Following IEEE p3652.1, a number of FL-related standards have been developed. In June 2020, China Mobile and AsiaInfo proposed "Federated Learning among Multiple NWDAF Instances" in the 3GPP R17 standard proposal TR23.700-91, introducing federated learning into 5G networks. In March 2021, China Telecom led a working group for IEEE P2986 "Recommended Practice for Privacy and Security for Federated Machine Learning", which focuses on the security and privacy of FL frameworks. %In November 2021, AsiaInfo led the working group of IEEE P3127 "Guide for an Architectural Framework for Blockchain-based Federated Machine Learning", which combines federated learning with blockchain. 
In June 2021, the ITU-T "Management Requirements for Federated Machine Learning Systems" international standard proposal submitted by Beijing University of Posts and Telecommunications was approved. %Support the management of future distributed intelligent computing networks represented by federated machine learning.
In general, these international standards are mainly based on FL frameworks and functions in the early stage. %In June 2022, IEEE P3187 "Guide for Framework for Trustworthy Federated Machine Learning" initiated by China Telecom was approved. This guide provides a reference framework for trustworthy Federated Machine Learning. 
These standards cover the classification of vertical federated learning and describe the relevance of vertical federated learning in the process of project establishment and formulation. % \yang{add a few sentences on VFL covered in these standards}

Current standardization efforts of federated learning framework helped to lay the foundation of basic functionalities, architectures and performance evaluations for developing FL frameworks. As more privacy-preserving platforms are deployed in applications,  production-level performance and efficiency, inter-platform connectivity and compatibility, as well as deep integration with applications will become the crucial challenges that drive the future development of standardization. %  At present, they have gradually begun to expand from basic functional standards to product performance and security, as well as cross-integration with other technologies.

%\subsubsection{Real-world Use Cases}
\subsection{Advertising}

In the field of digital advertising, the development of the advertising industry has long been accompanied by security and privacy problems of data use. %With the rapid development of the mobile Internet and the comprehensive popularity of mobile devices, a large amount of data has been generated, which leads to an increasing demand for legal, compliant, safe and efficient data cooperation among advertising enterprises. 
The digital advertising industry is complicated, involving advertisers, advertising platforms, consumers and other parties. Data is usually distributed in different companies as well as individual mobile devices, forming various data silos. Vertical federated learning is widely used to solve the data collaboration problem among companies in this field. Advertisers and advertising platforms, such as social media companies often have different attributes of the same group of people. Advertisers have customers' purchase behaviors and social media has customers' profiles and social preferences etc. Therefore it is natural for them to build data collaboration models via VFL. 


%Sun et al.\cite{sun2021defending} designed a vertical federation framework based on confrontation training and verified it on large-scale industrial online advertising data to ensure the privacy of input.


VFL has been applied to many real-world uses cases in recommendation and advertising. For example, ByteDance uses tree-based VFL and Fedlearner to greatly improve their advertising efficiency \cite{cai2020Bytedance}. Based on the 9N-FL framework and the VFL, JD has established a joint model for advertising, which has promoted the cumulative increase of both parties' income by 20\% \cite{Hou2021JD}. Tencent applies Angel PowerFL platform and VFL to the federation between advertisers and advertising platforms to improve model accuracy\cite{tencent2021}.
Relying on its open-sourced project EFLS \cite{EFLS2022}, Alimama has helped many companies with branding tasks. Some of the downstream tasks have achieved a 15\% increase in brand ROI within 2 months, and the business has improved significantly\cite{Alimama2022}. In addition, based on the trusted intelligent computing service framework (TICS), Huawei also applies vertical federated learning to advertising\cite{Wu2022Huawei}.

\subsection{Finance}

In the financial field, marketing and risk control are two important tasks. Since banks often lack the necessary information for comprehensive risk evaluation, they resort to external data sources to improve model performance. With the increasing requirements for data privacy protection and the promulgation of relevant laws and regulations in many countries, it has become difficult and even prohibitive to acquire alternative data for credit risk control, such as information about individuals' qualifications, purchasing ability, purchasing preferences etc., which are often available at e-commerce platforms, and social media companies. In this context, vertical federated learning is used to solve the joint modeling problem across institutions. \cite{long2020openbanking} discusses the applications and open challenges for FL in open banking. New approaches have been rapidly developed to adapt VFL frameworks to finance. For example, a gradient-based method for traditional scorecard model training is proposed in\cite{zheng2020vertical}, which is based on logistic regression with bounded constraints (LRBC) to obtain optimal performance.  In \cite{chen2021homomorphic}, a secure large-scale sparse logistic regression algorithm is designed by using homomorphic encryption and secret sharing, and is applied to financial risk control, which greatly improves the modeling efficiency. \cite{hu2022vertical} uses vertical logistic regression (VLR) trained with mini-batch gradient descent, and proposes that this method can be well applied in the financial field. 
%\yang{add more use cases. For example, Webank uses FedRiskCtrl, a VFL framework to connect to more micro and small enterprises \cite{cheng2020federated}. }
WeBank uses customers' credit data and invoice information from partner companies to jointly build a risk control model, improving the AUC of the risk control model for small and micro enterprises \cite{cheng2020federated}. In addition, Industrial and Commercial Bank of China used vertical federated learning to establish fraud account identification model with other institutions, which improved the accuracy rate of the joint model by 38.3\%, the accuracy rate by 28.9\% and the recall rate by 37.2\% compared with the independent model\cite{Cheng2022DigitalEra}. %\yang{what is the url? I can't find this ref.}

Similar scenarios and opportunities are applicable to insurance industry. \cite{Wang2019Shapley} provides an overview of use cases of FL in insurance industry. In general, with the continuous improvement of the security and efficiency of vertical federated learning algorithms, there will be more and more applications in the financial field. 

\subsection{Healthcare} 

In the field of smart medical care, the accuracy of machine learning model prediction depends on the quality and quantity of available medical data. However, due to the strict privacy requirement in medical field, it becomes very difficult to collect and share medical data scattered in various hospitals. The vertical federated learning framework provides an effective solution for the application scenarios in which the data features of a single medical institution are not rich enough, and data from more medical institutions need to be combined\cite{price2019privacy,lee2019discovery}.

Applied research of VFL to medical scenarios have been very active. A privacy-preserving logistic regression is proposed in \cite{hu2022vertical} and applied to clinical diagnosis. Chen et al\cite{chen2020vafl}, proposed an asynchronous vertical federated learning framework and verified the effectiveness of the framework on the public health care dataset MIMIC-III. In\cite{rooijakkers2020convinced}, the authors applied VFL to cancer survival analysis to predict the likelihood of someone surviving time after diagnosis and to analyze which features might be associated with the chance of survival.
In\cite{cha2021implementing}, the authors propose a method for VFL using autoencoders and predict hearing impairment after surgery based on the vestibular schwannoma dataset.
Song et al.\cite{song2021federated} applied VFL to the joint modeling between mobile network operators (MNOs) and health care providers (HP), and improved HP user classification in health care recommendations using MNO data. 

\subsection{Emerging applications}
Besides applications in Advertising, Finance, and Medical field, there are also emerging applications which exploit VFL for data mining and discovering novel data utilization in fields such as electric vehicles, wireless communications. For example, Teimoori et al.\cite{teimoori2022secure} proposed a secure recommendation system based on VFL, which is used to locate the charging pile for electric vehicles while protecting data privacy. \cite{Solmaz2020wireless} discussed the opportunities for VFL to be utilized in 5G wireless networks, e.g., for access mobility management
function (AMF) and session management function
(SMF) in the core network. \cite{zhang2020radionetworks} proposed VFL-based cooperative sensing for cognitive radio networks. \cite{hashemi2021optical} developed a VFL framework for optical network disaggregation. \cite{liu2021smartgrid} applied VFL to collaborative power consumption predictions in smart grid applications. \cite{ge2021failureprediction} proposed SVM and Random Forest modeling in both VFL and HFL scenarios for predicting failures in intelligent manufacturing. 


%\yang{any other interesting cases? e.g. covid-19 related, government related? }



%\subsubsection{Recommendation Systems}


==> dataset.tex <==
\section{Datasets}\label{dataset}

% We surveyed datasets that are commonly used in VFL works and categorize them into six groups, namely Finance, Medical, Citation, Advertising, Vehicle Signal and others. We list these datasets in Table \ref{tab:dataset}. We refer readers to the survey work~\cite{wu2021gnnsurvey} for more graph datasets.
% \yang{move footnotes to references to make it consistent.}
% \yan{may expand table 11 if time permitted.}
We list datasets commonly used in current VFL works in Table \ref{tab:dataset}. Most of the datasets used in VFL research are tabular datasets from Finance, Healthcare, and Advertising. This manifests that, on the one hand,  VFL has a broad range of applications in the three fields. On the other hand, tabular datasets dominate VFL research for their convenience in forming multi-party scenarios in VFL, indicating that we are short of research datasets of diverse types (e.g., image, text, or video). In addition, only NUSWIDE and Vehicle datasets consist of multi-modal features that can naturally simulate the two-party VFL scenario. Other datasets listed in Table \ref{tab:dataset} are adopted from existing machine learning research works, and there is no established way for VFL researchers to partition these datasets for VFL research. Therefore, facilitating industrial applications and academic research in the VFL area calls for practical datasets and high-quality benchmarks. 

% Regarding the evaluation metrics, top-1 accuracy is usually used for evaluating multiclass classification tasks, e.g. NUSWIDE, while Area under Curve (AUC) and F1-Score are adopted for imbalanced binary classification tasks, such as Avazu and Criteo etc.


% \begin{table*}[ht!]
% \centering
% %\renewcommand\thempfootnote{\arabic{mpfootnote}}
% %\begin{minipage}{\textwidth}
% % \footnotesize
% \caption{Commonly used datasets in VFL.\yang{change "Mixed" to specifics.e.g "text+image". "feature" column is not clear, what is "+","$\times$" mean, should be consistent. why unfilled blanks?}}
% \begin{tabular}{c|c||c|c|c|c|c}
% % \toprule[1.2pt]
% \hline
% \\[-1em]
% Category & Dataset & Data Type & Size & Feature & \# Classes & Description \\
% \hline
% \hline
% \multirow{5}*{\shortstack{Finance}} & Income~\cite{kohavi1996scaling} & Tabular & 48842 & 14 & 2 & Demographics and income features \\ %\footnote{\url{https://archive.ics.uci.edu/ml/datasets/adult}}
% \cline{2-7}
% \\[-1em]
% ~ & Bank~\cite{moro2014data} & Tabular & 41188 & 20 & 2 & Demographics and economic features \\ %\footnote{\url{https://archive.ics.uci.edu/ml/datasets/bank+marketing}}
% \cline{2-7}
% \\[-1em]
% ~ & Credit Card~\cite{yeh2009comparisons} & Tabular & 30000 & 24 & 2 & Demographics and payments  \\ %\footnote{\url{https://archive.ics.uci.edu/ml/datasets/default+of+credit+card+clients}}
% \cline{2-7}
% \\[-1em]
% ~ & Give Me Some Credit~\cite{givemesomecredit} & Tabular & 150K & 10 & 2 & Financial features  \\
% \hline
% \multirow{5}*{\shortstack{Medical}} & BHI~\cite{bhi} & Image & 277524 & 50$\times$50$\times$3 & 2 & Medical images \\
% \cline{2-7}
% \\[-1em]
% ~ & CheXpert~\cite{irvin2019chexpert} & Image & 65240 & 320$\times$320$\times$3? & 2  & Medical images \\
% \cline{2-7}
% \\[-1em]
% ~ & MIMIC III~\cite{johnson2016mimic} & Tabular & 40K+ &  &  & Medical records \\
% \cline{2-7}
% \\[-1em]
% ~ & Breast Cancer~\cite{street1993nuclear}  & Tabular & 569 & 30 & 2 & Breast tumor features \\ \cline{2-7}
% \\[-1em]
% ~ & Diabetes~\cite{smith1988using} & Tabular & 400 & 10 & 2  & Patient records \\ %\footnote{\url{https://archive.ics.uci.edu/ml/datasets/diabetes}}
% \hline
% \multirow{3}*{\shortstack{Citation}} & Cora~\cite{sen2008collective} & Graph & 2708/5429 & 1433 & 7 &  Citation network \\
% \cline{2-7}
% ~ & Citeseer~\cite{sen2008collective} & Graph & 3327/4732 & 3703 & 6 &  Citation network \\
% \cline{2-7}
% ~ & PubMed~\cite{sen2008collective} & Graph  & 19717/44338 & 500 & 3 & Citation network \\
% \hline
% \multirow{2}*{\shortstack{Advertising}} & Avazu~\cite{avazu} & Tabular & 1M+ & 26 + 13 & 2 &  Click-through data  \\
% \cline{2-7}
% ~ & Criteo~\cite{criteodata} & Tabular & 1M+ & 14 + 8 & 2 & Click-through data \\
% \hline
% \\[-1em]
% \multirow{2}*{\shortstack{Vehicle\\Signal}} & Vehicle~\cite{duarte2004vehicle} & Tabular & 50K & 50 + 50 & 3  & Acoustic and seismic signals \\ %\footnote{\url{https://www.csie.ntu.edu.tw/~cjlin/libsvmtools/datasets/}}
% \cline{2-7}
% \\[-1em]
% ~ & Drive~\cite{Dua2019} & Tabular & 58509  & 48 & 11  & Electric current drive signals\\
% \hline
% \multirow{7}*{\shortstack{Others}} & Cover type~\cite{blackard1999comparative} & Tabular & 581012 & 54 & 7 & Digital spatial data \\ 
% \cline{2-7}
% \\[-1em]
% ~ & NUSWIDE~\cite{nus-wide-civr09} & Tabular & 50K+ & 1000 + 634 & 10  & Tags and image descriptors \\
% \cline{2-7}
% ~ & Handwritten~\cite{van1998handwritten} & Tabular & 2000 & 649 & 10 & Handwritten digit features \\
% \cline{2-7}
% \\[-1em]
% ~ & Modelnet~\cite{wu20153d} & Image & 20K+ & 224$\times$224$\times$3 & 40 & Multi-views of 3D objects  \\
% \cline{2-7}
% ~ & Yahoo Answers~\cite{yahoo} & Text & 1.46M &  & 10  & Corpus of questions and answers \\
% \cline{2-7}
% \\[-1em]
% ~ & News20~\cite{keerthi2005modified} & Text & 19928 &  & 20 &  Newsgroup documents \\ %\footnote{\url{https://www.csie.ntu.edu.tw/~cjlin/libsvmtools/dat
% \cline{2-7}
% ~ & Epsilon~\cite{epsilon} & Tabular & 500K & 2000 & 2 & Synthetic data \\
% \hline
% \hline
% \end{tabular}
% %\end{minipage}
% \label{tab:dataset}
% \end{table*}
% \end{savenotes}

% \begin{savenotes}
\begin{table*}[ht!]
\centering
%\renewcommand\thempfootnote{\arabic{mpfootnote}}
%\begin{minipage}{\textwidth}
\footnotesize
\caption{Commonly used datasets in VFL. In the Size column, the number represents the total amount of samples of each dataset. For the three graph datasets, the number on the left of / represents the number of nodes, while the number on the right represents the number of edges. }
% \yang{change "Mixed" to specifics.e.g "text+image". "feature" column is not clear, what is "+","$\times$" mean, should be consistent. why unfilled blanks?}
\begin{tabular}{c||c|c|c}
% \toprule[1.2pt]
\hline
\\[-1em]
Dataset & Data Type & Size & Description \\
\hline
\hline
 Income~\cite{kohavi1996scaling} & Tabular & 48842 & Demographics and income features \\ %\footnote{\url{https://archive.ics.uci.edu/ml/datasets/adult}}
\hline
\\[-1em]
 Bank~\cite{moro2014data} & Tabular & 41188 & Demographics and economic features \\ %\footnote{\url{https://archive.ics.uci.edu/ml/datasets/bank+marketing}}
\hline
\\[-1em]
 Credit Card~\cite{yeh2009comparisons} & Tabular & 30000 & Demographics and payments  \\ %\footnote{\url{https://archive.ics.uci.edu/ml/datasets/default+of+credit+card+clients}}
\hline
\\[-1em]
Give Me Some Credit~\cite{givemesomecredit} & Tabular & 250000 & Debt features  \\
\hline
\\[-1em]
 MIMIC III~\cite{johnson2016mimic} & Tabular & 42276 & Medical records \\
\hline
\\[-1em]
Breast Cancer~\cite{street1993nuclear}  & Tabular & 569& Breast tumor features \\ 
\hline
\\[-1em]
 Diabetes~\cite{smith1988using} & Tabular & 400  & Patient records \\ %\footnote{\url{https://archive.ics.uci.edu/ml/datasets/diabetes}}
\hline
Avazu~\cite{avazu} & Tabular & 4M &  Click-through data  \\
\hline
\\[-1em]
 Criteo~\cite{criteodata} & Tabular & 4.5M & Click-through data \\
\hline
\\[-1em]
Vehicle~\cite{duarte2004vehicle} & Tabular & 98528 & Acoustic and seismic signals \\ %\footnote{\url{https://www.csie.ntu.edu.tw/~cjlin/libsvmtools/datasets/}}
\hline
\\[-1em]
 Drive~\cite{Dua2019} & Tabular & 58509 & Electric current drive signals\\
\hline
 Cover type~\cite{blackard1999comparative} & Tabular & 581012 & Digital spatial data \\ 
\hline
\\[-1em]
 NUSWIDE~\cite{nus-wide-civr09} & Tabular & 269648 & Image and the associated tags from Flickr \\
\hline
\\[-1em]
Handwritten~\cite{van1998handwritten} & Tabular & 2000 & Handwritten digit features \\
\hline
\\[-1em]
 Epsilon~\cite{epsilon} & Tabular & 500000 & Synthetic data \\
\hline
\\[-1em]
BHI~\cite{bhi} & Image & 277524 & Medical images \\
\hline
\\[-1em]
CheXpert~\cite{irvin2019chexpert} & Image & 65240  & Medical images \\
\hline
\\[-1em]
Modelnet~\cite{wu20153d} & Image & 20000  & Multi-views of 3D objects  \\
\hline
 Cora~\cite{sen2008collective} & Graph & 2708/5429 &  Citation network \\
\hline
Citeseer~\cite{sen2008collective} & Graph & 3327/4732 & Citation network \\
\hline
 PubMed~\cite{sen2008collective} & Graph  & 19717/44338 & Citation network \\
\hline
Yahoo Answers~\cite{yahoo} & Text & 1.46M & Corpus of questions and answers \\
\hline
\\[-1em]
News20~\cite{keerthi2005modified} & Text & 19928 &  Newsgroup documents \\ %\footnote{\url{https://www.csie.ntu.edu.tw/~cjlin/libsvmtools/dat
\hline
\hline
\end{tabular}
%\end{minipage}
\label{tab:dataset}
\end{table*}

==> system.tex <==

%\section{System Challenges}

